Towards a Framework to Manage Perceptual Uncertainty for Safe Automated Driving

Perception is a safety-critical function of autonomous vehicles and machine learning (ML) plays a key role in its implementation. This position paper identifies (1) perceptual uncertainty as a performance measure used to define safety requirements and (2) its influence factors when using supervised ML. This work is a first step towards a framework for measuring and controling the effects of these factors and supplying evidence to support claims about perceptual uncertainty.

==> conclusions.tex <==
\section{Conclusion} \label{sec:conclusion}

==> points.tex <==
\section{Analyzing sources of uncertainty} \label{sec:points}

%
%Assume we are using ML to implement a safety-critical perceptual function $F:X\rightarrow Y$ (e.g., a Pedestrian classifier). We can identify several sources of uncertainty:
%\begin{itemize}
%	\item (P1) Concept uncertainty: uncertainty about what is the specification of $F$
%	\item (P2) Sensory uncertainty: uncertainty in the sensory channel that produces inputs of type $X$ 
%	\item (P3) Labeling uncertainty: uncertainty about whether the dataset is correctly labeled wrt to $F$
%	\item (P4) Domain uncertainty: uncertainty about whether the dataset is representative of input distribution of $F$ during operation
%	\item (P5) Model uncertainty: uncertainty about whether the trained model correctly represents $F$
%\end{itemize}
%
%
%Reducing P5 is the goal we wish to attain and this is related to reducing the preceding sources of uncertainty. [Discuss these connections] 


In this section, we consider the research questions that must be addressed to realize an uncertainty-oriented view of perception safety. 

We can ask the following
\begin{itemize}
	\item (RQ1) What are the sources of uncertainty?
	\item (RQ2) How to measure and represent uncertainty levels?
	\item (RQ3) How are sources of uncertainty related?
	\item (RQ4) How can the uncertainty be reduced or mitigated?
	\item (RQ5) What evidence is needed to support uncertainty claims? 
\end{itemize}

\subsection{(RQ1) What are the sources of uncertainty?}
In Sec.~\ref{sec:perunc} we proposed a generic characterization of the different facets of perceptual component development (Fig.~\ref{??}). This allowed us to systematically identify the different sources of uncertainty that contribute to perceptual uncertainty. A generic characterization is useful methodologically because it allows specific techniques and tools to be developed to address particular sources of uncertainty.
Particular projects may vary. 

\subsection{(RQ2) How to measure and represent uncertainty levels?}
As discussed in Sec.~\ref{sec:perunc}, ideally, we assume uncertainty is expressed as a probability distribution over a set of possible values. In some cases, the set of values is clear. For example, the sensor uncertainty (U6) of a monochrome camera pixel can range over 256 pixel values while labeling uncertainty (U7) can be measured over the set of possible labeling outcomes that could be made. In other cases, uncertainty is more qualitative.
For example, assessing conceptual uncertainty (U1) may involve identifying specific examples that are particularly difficult to classify and providing reasons for the difficulty. Here the objective is to estimate the probability of encountering such examples in the domain. 

Another important issue is how and when uncertainty is detected and measured. In general there is a preference for identifying uncertainty at development time and reducing or mitigating it to achieve an acceptable level. In practice, this may not be completely possible [why?] and run-time monitoring can compensate. For example, \emph{confidence} measures (e.g., Bayesian deep learning~\cite{??}) can be used to provide a run-time measure of perceptual uncertainty in perception component output. Low confidence input samples can be collected for subsequent analysis to diagnose the specific source of the uncertainty. Novelty detection methods have been proposed to detect out-of-distribution inputs (i.e., outliers). For example, the training dataset can be used without labels to train an autoencoder to identify the characteristics of the dataset. At run-time, new inputs are checked for their similarity to the dataset (i.e., their novelty) by checking how well the autoencoder can reconstruct them~\cite{??}. The frequency of novel inputs encountered at run-time is a measure of operational domain uncertainty (U9).


\subsection{(RQ3) How are sources of uncertainty related?} \label{sec:depend}
Sources of uncertainty may be interdependent. Since the total perceptual uncertainty
for a particular perception component is an aggregate of the various uncertainty sources, understanding the dependencies between the sources
is crucial for determining how to assessing whether the target acceptable level of uncertainty has been achieved. 
Fig.~\ref{f:uncertdepend} provides a preliminary high level view of the dependencies. Some examples: sensor uncertainty (U6) causing noisy samples can lead to greater labeling uncertainty (U7) due to increased confusion for human labelers; higher conceptual uncertainty (U1) makes selecting adequate training samples more difficult leading to more training selection uncertainty (U4) and this increases the likelyhood of operational domain uncertainty (U9); and, there is more concept adequacy uncertainty (U2) when there is increased conceptual uncertainty (U1) because it is more difficult to be sure the concept definition meets requirements if the concept itself is unclear.	

The details of the dependencies between different sources of the uncertainty must be determined. This includes the direction of dependency, the degree of dependency and the extent to which the dependency can be formalized. For example, if sensor uncertainty and labeling uncertainty are both represented as a probability distributions, can the relationship between these distributions be estimated?   

\begin{figure} [h]
	\centering{
		%\vspace{-0.2in}
		\includegraphics[width=.8\textwidth]{images/uncertdepend.pdf}}
	%\vspace{-0.2in}
	\caption{Dependencies between sources of uncertainty that contribute to perceptual uncertainty.}
	%\vspace{-0.15in}
	\label{f:uncertdepend}
\end{figure}

\subsection{(RQ4) How can the uncertainty be reduced or mitigated?}
Uncertainty that is identified to be higher than acceptable must be reduced, or, if reduction is not possible, mitigated.
Table~\ref{t:reduce} gives examples of techniques that can be used to reduce or mitigate sources of uncertainty. 
A goal of this research is to provide a catalog of such techniques and to identify gaps where new techniques are needed.


\begin{table}
	\caption{Examples of techniques to reduce or mitigate uncertainty.} \label{t:reduce}
\begin{tabular}{|p{4in}|l|}
	\hline
	{\bf Technique} & {\bf Source} \\
	\hline
	Use rigorous dataset requirements using techniques -- e.g., from black-box software testing such as input domain partitioning~\cite{ammann2016introduction}.& U1,U2,U4, U9 \\
	\hline
	Identify behavioral constraints including assumptions, pre/post conditions, invariants and equivariants. & U1-U4, U9 \\
	\hline
	Use techniques to improve ML interpretability -- e.g., generating explanations (e.g., ~\cite{ribeiro2016should}). & U8 \\
	\hline
	Actively improve situation characteristics -- e.g., using lighting to increase poor illumination. & U5 \\
	\hline
	Automate labeling through instrumentation (e.g., installing V2X modems) or unsupervised learning. & U7 \\
	\hline
	Use data augmentation techniques to produce new labeled data from existing samples. & U4, U8 \\
	\hline
	Collect and analyze outliers using novelty detection~\cite{??}. & U1, U4, U9 \\
	\hline
	Use sensor fusion to mitigate limitations of individual sensors. & U6 \\ 
	\hline
	Detect and manage ODD violations~\cite{colwell18} to avoid novelty.& U9 \\
	\hline
\end{tabular}
\end{table}



\subsection{(RQ5) What evidence is needed to support uncertainty claims?} 
As part of a rigorous safety assurance process, claims regarding uncertainty must be supported by evidence and documented in a safety case.
One type of uncertainty claim is concerned with completeness -- e.g., that all sources of uncertainty have been identified. Our proposed 
taxonomy of uncertainty sources provides reference model and can be used as evidence for such a claim. However, the sources in the taxonomy 
are ``categorical'' and are is intended to 
be refined further for particular perception components. For example, refining situation uncertainty (U5) for a pedestrian detector intended to operate on a particular set of roads involves identifying the different ways that structural aspects of those roads can limit observability of pedestrians. Thus, additional completeness claims must be made about these refinements and evidence of analytical effort must be provided. 

Another kind of uncertainty claim is that the level uncertainty is limited to some bounds. When this is applied to perceptual uncertainty as 
a whole, then an argument must be given about how the claims about different sources of uncertainty contribute to it. This is supported by 
the dependency analysis discussed in Sec.~\ref{sec:depend}. Claims about the individual sources of uncertainty require diverse forms of evidence
depending on the source. For example, bounds on sensor uncertainty (U6) may appeal to bench testing results while bounds on model uncertainty (U8) 
can be supported by Bayesian estimates of uncertainty in model parameters given the training data~\cite{malinin2018predictive}. 
	


%\subsection{Approaches to addressing research questions}
%\begin{itemize}
%	\item Runtime vs. Devtime detection
%	\item Architectural techniques for reduction and mitigation
%	\begin{itemize}
%		\item ensemble methods for reducing error rate
%		\item simplex
%		\item safety envelope
%		\item tracking and propagating uncertainty - make downstream components ``uncertainty aware''
%		
%		\begin{itemize}
%			\item representing classification uncertainty by finding highest class in ontology
%			\item representing uncertainty of real values using a distribution (e.g., Gaussian)
%		\end{itemize}
%	\end{itemize} 
%\end{itemize}

% -- Old begins here --
% 
%\subsection {(P1)  Concept uncertainty}
%Spanfelner et al.~\cite{spanfelner2012challenges} point out that functionality required for automation such as perception may not be completely specifiable. For example, what is the complete set of necessary and sufficient conditions for recognizing a pedestrian? There is evidence that humans use both rules and examples for perception of such concepts~\cite{rouder2006comparing}. This is a clear motivation for using ML rather than programming for such functions. 
%
%However, a specification that uses examples is necessarily incomplete because there remains uncertainty about cases not covered. Furthermore, concepts like ``Pedestrian'' are human constructs and thus, the ground truth for their recognition come from humans. However, people can disagree on some cases.  Thus, although we may be able to reduce the epistemic uncertainty about the concept by doing more analysis, there is a limit to this process and some aleatoric uncertainty remains. We have argued~\cite{salay18} that the irreducibility of the uncertainty about the concept specification is a key obstacle in ISO 26262 and other safety standards based on the \name{V} model because they assume that component behaviour can be fully specified~\cite{spanfelner2012challenges,bhattacharyya2015certification}.
%
%Analysis to reduce uncertainty (RQ2) includes identifying new rules and requirements on the dataset of examples. Rules include assumptions (e.g., images have good lighting), pre/post conditions (e.g., pedestrians $<$ 9 feet tall), invariants and equivariants (e.g., a rotated pedestrian image is still a pedestrian). Dataset requirement analysis can be based on techniques from black-box software testing such as input domain partitioning~\cite{ammann2016introduction}. For example, the input domain of a pedestrian classifier could be partitioned by age category, pose (e.g., standing, leaning, etc.), clothing type, etc. The data requirements can specify the relative numbers of samples that should come from each partition to ensure coverage and representativeness of the sample data and reduce domain and model uncertainty. The aleatoric uncertainy can be mitigated to a degree by identifying an authorative source for the gold standard (RQ3). This is more feasible for more regulated concepts such as ``Vehicle'' [Definition from NIST?] than colloquial concepts like ``Pedestrian''.  For these concepts, a specific identified human ``expert'' can be used as the gold standard. 
%
%%\begin{itemize}
%%	\item (RQ2) The epistemic uncertainty is reduced by doing more analysis of F.   
%%	\item The aleatoric uncertainty here occurs when F is not completely specifiable as is the case with classification into human-created categories (e.g. pedestrian). This is a motivation for using ML rather than programming.
%%	\begin{itemize}
%%		\item (RQ3) Mitigated using a Partial Specification~\cite{salay18}
%%		\item (RQ3) Mitigated using a human can be a surrogate for a specification since perception represents human competency
%%	\end{itemize}	
%%\end{itemize}
%
%\subsection {(P2)  Sensory uncertainty}
%Sensed information may be limited by physical object and scene properties (object salience, viewpoint, occlusions, illumination, atmospheric visibility, distance, clutter, crowding, etc.) and sensor properties (sensitivity, noise, range, etc.). The more limited information about the target in the sensory data, the higher the uncertainty about the target. Some sources sensory uncertainty such as sensor noise can be directly measured through sensor testing and a noise model can be expressed as a probability distribution (RQ1). Sensor noise is typically considered to be aleatoric but even this could be reducible if the sensor can be replaced by a less noisy sensor (RQ2). The noise model can be used to mitigate the effects of the uncertainty (RQ3). For example, a Kalman Filter~\cite{??} uses Gaussian noise models of observations to fuse different sensor inputs and improve state estimates. 
%Other sources of sensory uncertainty can be reduced (RQ2) by manipulating the scene properties - e.g., moving to change viewpoint, using lighting to increase illumination, etc. 
%
%
%
%\subsection {(P3) Labeling uncertainty}
%The dataset must be labeled before use for training or testing and there can uncertainty about the correctness of the labels. Human labelers may assign varying labels because of concept or sensory uncertainty; but even if these sources of uncertainty are low, humans may still make mistakes - e.g., a human may accidentally select the wrong target in the scene image when labeling. Label uncertainty can be reduced through automation (RQ2). One approach is to instrument the physical scene (e.g., installing V2X modems on targets; see dashed arrow in Fig.~\ref{f:pertri}), but this is often costly or impractical.
%Another approach is to use data augmentation techniques to produce new labeled data. Invariants and equivariants from the concept specification can be used to generate new labeled examples from existing ones. For example, Generative Adversarial Networks (GANs) have been used to implement transformations that can convert a scene into another one with different attributes such as adding snow, rain, etc.~\cite{liu2017unsupervised}. Wong et al. investigate the benefit of different data augmentation techniques~\cite{wong2016understanding}. But while data augmentation produces new labeled data automatically, if the input data is incorrectly labeled, so will the new data. Thus, data augmentation should only be applied where there is already a low uncertainty about label correctness. 
%%\begin{itemize}
%%	\item Despite (1), the epistemic uncertainty here can be low because perception is a human competency (unlike e.g., cancer diagnosis). Although labeling is costly.
%%	\item There may be aleatoric uncertainty for some inputs due to, e.g., irreducible noise in inputs, lack of consensus on classification, etc.	
%%\end{itemize}
%
%\subsection {(P4) Domain uncertainty}
%The specification incompleteness due to concept uncertainty means that the perception component is trained on subset of the input domain. Domain uncertainty is the lack of knowledge about how representative this subset is of the inputs actually encountered during operation. 
%For example, training did not cover pedestrians using walking aids or pedestrians in unusual poses, such as lying on the pavement. This epistemic uncertainty can be reduced (RQ2) at development time by rigorously analyzing the operational input domain to produce dataset requirements as discussed above for concept uncertainty. 
%These ensure that there is adequate coverage in the dataset and, crucially, that there is adequate representation of rare but high risk inputs. 
%
%During operation, domain uncertainty can be detected (RQ1) by using novelty detection methods to identify
%out-of-distribution inputs (i.e., outliers). For example, the training dataset can be used without labels to train an autoencoder to identify the characteristics of the dataset. At run-time, new inputs are checked for their similarity to the dataset (i.e., their novelty) by checking how well the autoencoder can reconstruct them~\cite{??}. Identified outliers can be tracked to subsequently update the dataset and reduce domain uncertainty (RQ2) and they can also be used to mitigate domain uncertainty (RQ3) by providing a safer (but more conservative) way of handling them using a Simplex~\cite{sha2001using} style architectural pattern. 
%
%An exacerbating factor in domain uncertainty is \emph{distributional shift} -- the gradual
%change in the operational distribution over time~\cite{amodei2016concrete}. For example, slowly changing facets of a city-scape can eventually affect the validity the trained model. This may be detected (RQ1) by tracking the frequency with which outliers occur and addressed by redeveloping the dataset when this exceeds some threshold. 
%
%Finally we consider an approach to mitigating domain uncertainty (RQ3) by controlling the operational environment itself. ADSs are typically only intended to operate safely within a particular Operational Design Domain (ODD) -- a set of assumed conditions on the environment and driving modes~\cite{standard2014j3016}. For example, the ODD may specify that the weather must be clear and no highway driving is permitted. Such conditions
%clearly put bounds on the operational domain and provide a basis for dataset requirements. However, for this to be effective, the ODD must be enforced
%during ADS operation and specialized architectural strategies can be used to address this~\cite{colwell18}.   
%
%
%
%%Domain uncertainty is 
%%due to many factors. Inadequate domain coverage of the dataset 
%%\begin{itemize}
%%	\item The epistemic uncertainty here is due to
%%	\begin{itemize}
%%		\item inadequate domain coverage of training data
%%		\begin{itemize}
%%			\item (RQ1) detected by doing domain analysis (e.g., partitioning)
%%			\item (RQ2) reduced by and adding training examples for the gaps
%%		\end{itemize}
%%		\item under-representation of higher risk inputs
%%		\begin{itemize}
%%			\item (RQ1) detected by doing risk analysis
%%			\item (RQ2) reduced by and adding training examples for the gaps
%%		\end{itemize}
%%		\item inadequate representativeness of the operational distribution by the dataset
%%		\begin{itemize}
%%			\item (RQ1) detected by monitoring the input distribution during operation for differences from expectation (e.g., using \emph{novelty detection})
%%			\item (RQ2) reduced by adjusting the dataset correspondingly
%%			\item (RQ3) mitigated by fault tolerance such as simplex
%%		\end{itemize}
%%		
%%	\end{itemize}	
%%	\item Theoretically, the epistemic uncertainty decreases as training data is increased, and, due to PAC guarantees ensures that the trained model will eventually converge to F. But practically, this guarantee cannot be used due to the large number of samples it requires Thus, the careful choice of dataset (as described above) is the determiner of the rate of decrease
%%	\item The aleatoric uncertainty here is due to the fact that there is a time delay between training/testing and operational distribution and thus a quickly changing operational distribution cannot be accommodated
%%	
%%\end{itemize}
%
%\subsection {(P5) Model uncertainty}
%\begin{itemize}
%	\item The epistemic uncertainty here is due to
%	\begin{itemize}
%		\item overfitting of the model to the training data
%		\begin{itemize}
%			\item (RQ1) detected by validation activities
%			\item (RQ2) reduced by increasing diversity in the dataset, adding prior knowledge to the  model (e.g., via regularization) or changing the hyper-parameters
%		\end{itemize}
%		\item the model being too weak to represent F (underfitting)
%		\begin{itemize}
%			\item (RQ1) detected by error rate that cannot be adequately reduced
%			\item (RQ2) reduced by changing model type or hyper-parameters
%		\end{itemize}
%		\item even if (2) is addressed, the inability to determine what is correct behavior due to (1)
%		\begin{itemize}
%			\item (RQ2) reduced by reducing epistemic uncertainty in (1) and (2)
%		\end{itemize}
%		\item the dataset being insufficiently complete to correctly determine F
%		\begin{itemize}
%			\item (RQ1) detected by low confidence classification predictions during operation (e.g., using Bayesian \emph{confidence measure})
%			\item (RQ2) reduced by adding samples to the dataset for low confidence cases
%			\item (RQ2) reduced by increasing the dataset (by PAC learning) but practically speaking, the epistemic uncertainty in (3) and (4) must be reduced			
%		\end{itemize}
%		\item Lack of interpretability of the trained model. The question of interpretability can either be \emph{global} when applied to the entire trained model or \emph{local} when applied to individual inferences made by the model~\cite{guidotti2018survey}.
%		\begin{itemize}
%			\item (RQ2) reduced at the global level to support static verification by using more transparent general model types, such as Bayesian networks or rule-based models are recognized as being more transparent than others as are more specialized model types such as Deformable Part Models for predestrian detection~\cite{yan2013robust}. The focus of the research on non-transparent model types such as NNs or SVMs includes visualizations (e.g.,~\cite{vondrick2013hoggles}), rule extraction (e.g.,~\cite{martens2009decompositional}) and analyzing dependence of ouputs on inputs (e.g.,~\cite{goldstein2015peeking}).  
%			\item (RQ2) reduced at instance level (dynamic verification) by explanation generation - test passed for the right reason?, what is reason for test failure? Saliency mask which identifies the subset of the input features responsible for the prediction (e.g.,~\cite{mahendran2016salient}). Text based explanations produce natural language explanations of the model predictions features (e.g., ~\cite{hendricks2016generating}).
%		\end{itemize}
%		\item inadequate structural and domain coverage of the test data (for dynamic verification)
%		\begin{itemize}
%			\item (RQ1) Inadequate domain coverage detected by doing traditional domain analysis for software test suite design. Assessing structural coverage of ML models is a new field but recent results exist (e.g.,~\cite{sun2018testing}).
%			\item (RQ2) reduced by extending the dataset to address gaps
%		\end{itemize}
%					\item (RQ1) detected by analyzing the differences between the training and operational environments
%		\item (RQ2) reduced by replicating the operational environment as closely as possible when generating the dataset
%		
%	\end{itemize}
%	\item One source of aleatoric uncertainty is due to non-determinacy of the model (for model types that are probabilistic)
%	\item It is not clear whether aleatoric uncertainty applies here as it does with programmed software due to the undecidability of program correctness in general. [Is undecidability another kind of irreducible uncertainty since it is not stochastic?]
%\end{itemize}
%
%Finally, although complete behavioral specifications are not possible, partial specifications may still be.
%For example, if a pedestrian must be less than 9 feet tall, then
%this property can be used to filter out false positives.
%Such properties can be incorporated into the training process or checked on models
%after training (e.g.,~\cite{katz2017reluplex}). 
%Some of these recommendations may be addressed in a forth-coming OMG standard 
%relating to sensor and perception issues~\cite{ISO21448}.



